Fault-Tolerant Aggregation: Flow-Updating Meets Mass-Distribution

Flow-Updating (FU) is a fault-tolerant technique that has proved to be efficient in practice for the distributed computation of aggregate functions in communication networks where individual processors do not have access to global information. Previous distributed aggregation protocols, based on repeated sharing of input values (or mass) among processors, sometimes called Mass-Distribution (MD) protocols, are not resilient to communication failures (or message loss) because such failures yield a loss of mass. In this paper, we present a protocol which we call Mass-Distribution with Flow-Updating (MDFU). We obtain MDFU by applying FU techniques to classic MD. We analyze the convergence time of MDFU showing that stochastic message loss produces low overhead. This is the first convergence proof of an FU-based algorithm. We evaluate MDFU experimentally, comparing it with previous MD and FU protocols, and verifying the behavior predicted by the analysis. Finally, given that MDFU incurs a fixed deviation proportional to the message-loss rate, we adjust the accuracy of MDFU heuristically in a new protocol called MDFU with Linear Prediction (MDFU-LP). The evaluation shows that both MDFU and MDFU-LP behave very well in practice, even under high rates of message loss and even changing the input values dynamically.

==> _region_.tex <==
\message{ !name(intro.tex)}
\message{ !name(intro.tex) !offset(-2) }



\section{Introduction}

The distributed computation of algebraic aggregate functions is particularly challenging in settings where the processing nodes do not have access to global information such as the input size. A good example of such scenario is \SNs~\cite{akyildiz-survey,ravi-survey} where unreliable sensor nodes are deployed at random and the overall number of nodes that actually start up and sense input values may be unknown.
Even more challenging is that loss of messages between nodes or even node crashes are likely in such harsh settings. 
It has been proved~\cite{BGMGM:agg} that the problem of aggregating values distributedly in networks where processing nodes may join and leave arbitrarily is intractable.
Hence, arbitrary adversarial message loss also yields the problem intractable, but a weaker adversary, for instance a stochastic one as in \DNs~\cite{CPMS:dynRN}, is of interest.
In this paper, under a stochastic model of message loss, we study communication networks where each node holds an input value and the average of those values must be obtained by all nodes, none of whom have access to global information of the network~\footnote{Other algebraic aggregate functions can be computed in the same bounds using an average protocol~\cite{CPX:SNaggJournal, KDGgossip}.}.

A classic distributed technique for aggregation, sometimes called \defn{Mass Distribution}~(\MD)~\cite{FMT:agg}, works in rounds. In each round, each node shares a fraction of its current average estimation with other nodes, starting from the input values~\cite{KDGgossip, BGPSgossip, Chen09, CPX:SNaggJournal}. Details differ from paper to paper but a common problem is that, in the face of message loss, those protocols do not converge to a correct output.
Recently~\cite{ABJ:flowupdate, ABJ:flowupdatedyn}, a heuristic termed \defn{Flow Update} (\FU) addressed the problem assuming stochastic message loss~\cite{ABJ:flowupdate}, and even assuming that input values change and nodes may fail~\cite{ABJ:flowupdatedyn}.
The idea underlying \FU is to keep track of an aggregate function of all communication for each pair of communicating nodes, since the beginning of the protocol, so that a current value at a node can be re-computed from scratch in each round.
Empirical evaluation has shown that \FU behaves very well in practice~\cite{ABJ:flowupdate, ABJ:flowupdatedyn}, but  such protocols have eluded analysis until now.

%\parhead{Our Contributions}
In this paper, we introduce the concept of \FU to \MD. First, we present a protocol that we call \defn{Mass Distribution with Flow Update} (\MDFU). The main difference with \MD is that, instead of computing incrementally, the average is computed from scratch in each round using the initial input value and the accumulated value shared with other nodes so far (which we refer to as either \defn{mass shared}, or \defn{flow passed}). The main difference with \FU is that if messages are not lost the algorithm is exactly \MD, which facilitates the theoretical analysis of the convergence time under failures parameterized by the failure probability (or \defn{message-loss rate}).

\parhead{Our results}%The analysis shows the following.
We first leverage previous work on bounding the mixing time of Markov chains~\cite{SJ:count} to show that, for any $0<\xi<1$, the convergence time of \MDFU under reliable communication is 
$2\ln(n/\xi)/\Phi(G)^2$, 
where $\Phi(G)$ is the conductance of the underlying graph characterizing the execution of \MDFU on the network.
Then, we show that, with probability at least $1-1/n$,
for a message-loss rate $f < 1/\ln(2\Delta e)^3$, the multiplicative overhead on the convergence time produced by message loss is less than $1/(1-\sqrt{f\ln(2\Delta e)^3})$, and it is constant for $f\leq 1/(e(2\Delta e)^e)$, where $\Delta$ is the maximum number of neighbors of any node.
Also, we show that, with probability at least $1-1/n$, 
for any $0<\xi<1$, after convergence 
the expected average estimation at any node is in the interval $[(1-\xi)(1-f) \overline{v},(1+\xi)\overline{v}]$.
This is the first convergence proof for an \FU-based algorithm.

In \MDFU, if some flow is not received, a node computes the current estimation using the last flow received. Thus, in presence of message loss, nodes do not converge to the average and only some parametric bound can be guaranteed as shown. Aiming to improve the accuracy of \MDFU, we present a new heuristic protocol that we call \defn{MDFU with Linear Prediction} (MDFU-LP). The difference with \MDFU is that if some flow is not received a node computes the current estimation using an estimation of the flow that should have been received.

We evaluate \MDFU and \MDFULP experimentally and find that the performance of \MDFU is comparable to \FU and other competing algorithms under reliable communication. In the presence of message loss, the empirical evaluation shows that \MDFU behaves as predicted in the analysis converging to the average with a bias proportional to the message-loss rate\marginpar{Whereas \FU blah blah blah}. In a third set of evaluations, we observe that \MDFULP converges to the correct value very fast, even under high message loss rates. We also test \MDFU and \MDFULP under changing input values to verify that both tolerate dynamic changes in practice, in contrast to classic \MD algorithms, which need to restart the computation each time values are changed. 

\noindent\parhead{Roadmap}
In Section~\ref{sec:prelim} we formally define the model and the problem, and we give an overview of related work. Sections~\ref{sec:alg},~\ref{sec:ana}, and~\ref{sec:eval} include the details of \MDFU, its analysis, and its empirical evaluation, respectively. Finally, in Section~\ref{sec:vel}, we present the details of \MDFULP and its experimental evaluation. An evaluation of \MDFU and \MDFULP in a dynamic setting, where input values change over time, is left to the Appendix.



\message{ !name(intro.tex) !offset(-42) }

